Repairing Regressors for Fair Binary Classification at Any Decision Threshold

We study the problem of post-processing a supervised machine-learned regressor to maximize fair binary classification at all decision thresholds. By decreasing the statistical distance between each group's score distributions, we show that we can increase fair performance across all thresholds at once, and that we can do so without a large decrease in accuracy. To this end, we introduce a formal measure of Distributional Parity, which captures the degree of similarity in the distributions of classifications for different protected groups. Our main result is to put forward a novel post-processing algorithm based on optimal transport, which provably maximizes Distributional Parity, thereby attaining common notions of group fairness like Equalized Odds or Equal Opportunity at all thresholds. We demonstrate on two fairness benchmarks that our technique works well empirically, while also outperforming and generalizing similar techniques from related work.

==> packages.tex <==
\usepackage{bbm}
\usepackage{bm}
\usepackage{amsmath,amsthm}
\usepackage{algorithm}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{subcaption} % added by jess
\usepackage{dsfont} % added by jess
\usepackage{macros}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{nameref}
\usepackage{graphicx}
\usepackage[normalem]{ulem}
\usepackage{natbib}
\usepackage[abs]{overpic}
\usepackage{algorithmic}


% \usepackage{ulem} % Do not use this; use \looseness=-1 for danglers (Cooper)
\usepackage{hhline}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{enumitem}       % for resuming enumer


\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{example}{Example}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{fact}{Fact}[section]

==> sections/20_setup.tex <==
\vspace{-.2cm}
\section{Wasserstein Distance and Wasserstein Barycenters}
\label{sec:setting}
Before introducing our solution, we must present some necessary background on Wasserstein distance and Wasserstein barycenters; see \cite{Villani2008OptimalTO, ComputationalOptimalTransport, santambrogio2015optimal} for a more in-depth treatment. Readers familiar with optimal transport can skip this section on a first read of the paper. 
   

\paragraph*{Wasserstein Distance.} Informally, the Wasserstein distance captures the difference between probability measures by measuring the \textit{cost} of transforming one probability measure into the other.   In the special case when distributions are univariate, the Wasserstein distance has a nice closed form. 
\begin{definition}[Wasserstein Distance]
 For two measures $\mu_1, \mu_2 \in \Ppm{p}(\ospace)$ where $\dim(\ospace) = 1$
\vspace{-.1cm}
\begin{align}
\label{eq: wasserstein_def}
    \Wass_{p}^{p}(\mu_1,\mu_2) &= \int_{\ospace}|F^{-1}_{\mu_1}(q) - F^{-1}_{\mu_2}(q)|^p dq.
\end{align} 

\end{definition}
We can also define the Wasserstein distance using transport plans; this is commonly referred to as Monge's Formulation.  A transport plan is a  function $T \in \mc T$ where every function in $\mc T$ satisfies standard pushforward constraints, i.e, $T_{\#}\mu_1 = \mu_2$ such that $\mu_{2}(B) = \mu_1(T^{-1}(B))$ for all measurable $B \subseteq \ospace$.   
\begin{definition}[Wasserstein Distance \text{[Monge]}]
\begin{align}
\label{eq: wass_tp_def}
     \Wass_{p}^{p}(\mu_1,\mu_2) &= \inf_{T \in \mc T} \int_{\ospace}|q - T(q)|^p d\mu_1. 
\end{align}  
\end{definition}


In our specific case where $\ospace \subseteq \reals{}$ and Assumption \ref{assumption:wass} is satisfied, we know that these transport plans which solve Monge's formulation exist and we can define them in closed form.\looseness=-1 
\begin{remark}
\label{rem:transport_plan}
 The transport plan from $\mu_1 \rightarrow \mu_2$ which minimizes Eq. (\ref{eq: wass_tp_def}) is defined $T_1^2(x) = F^{-1}_{\mu_2}(F_{\mu_1}(x))$ for all $p \geq 1$ \cite[Remark 2.6]{santambrogio2015optimal}  
\end{remark}
\label{eq:transport_plan}

% Equivalently, we can define optimal transport using a transport function $T \in \mc T$ where every function in $\mc T$ satisfies standard pushforward constraints, i.e, $T_{\#}\mu_1 = \mu_2$ such that $\mu_{2}(B) = \mu_1(T^{-1}(B))$ for all measurable $B \subseteq \ospace$. 
% \begin{align}
% \label{eq: wass_tp_def}
%      \Wass_{p}^{p}(\mu_1,\mu_2) &= \inf_{T \in \mc T} \int_{\ospace}|q - T(q)|^p d\mu_1. 
% \end{align}  


% \begin{claim}
% \label{eq:transport_plan}
% In our specific case where $\ospace \subseteq \reals{}$ and Assumption \ref{assumption:wass} is satisfied, the transport plan from $\mu_1 \rightarrow \mu_2$ which minimizes Eq. (\ref{eq: wass_tp_def}) is defined $T_1^2(x) = F_{\mu_1}(F^{-1}_{\mu_2}(x))$ for all $p \geq 1$ \cite{santambrogio2015optimal}[Theorem 2.9]
% \end{claim}

\paragraph*{Wasserstein Barycenter.} The Wasserstein barycenter % \footnote{Originally introduced for $\Wass_2$  but later studied for other orders, like $\Wass_1$ (see, e.g., \cite{cuturi2014fast}).} 
is a weighted composition of two distributions, much like a weighted average or midpoint in the Euclidean sense; it provides a principled way to compose two measures. 
\begin{definition}[Wasserstein Barycenter]
\label{def:barycenter}
For two measures $\mu_1,\mu_2 \in \Ppm{p}(\ospace)$ their $\alpha$-weighted \textit{Wasserstein barycenter}\footnote{Although defined in \cite{agueh2011barycenters} for p=2, this definition for all $p\geq 1$ is widely accepted.} is denoted $\mu_\alpha$ and is computed
\begin{align}
\label{eq:barycenter}
\mu_\alpha \leftarrow \argmin_{\nu \in \Ppm{p}(\ospace)}  (1-\alpha)\Wass_p^p(\mu_1, \nu) + \alpha\Wass_p^p(\mu_2, \nu), 
\end{align}
and in the special case when $\alpha=\rho_\protp$ we write $\mu^*$.  
\end{definition}
\noindent To complete the weighted-average analogy, $\alpha$ behaves like a tunable knob: As $\alpha \rightarrow 0$ then $\mu_\alpha$ will appear more like $\mu_1$, and as $\alpha \rightarrow 1$ the more $\mu_\alpha$ will appear like $\mu_2$.  

As a consequence of this definition and Remark \ref{rem:transport_plan}, we can express the transport plan to a barycenter in closed form as well\footnote{Proof of this result can be found in the appendix.}. 
\begin{corollary}
\label{cor:barycenter_transport_plan}
Let $\mustar$ be the $\rho_\protp$-weighted barycenter of $\mu_\pa,\mu_\protp$ then the transport plan from $\mu_\pa \rightarrow \mustar$ (wlog) is computed 
 \begin{align*}
T_\pa^*(\omega) =  (\rho_\pa F_{\mu_\pa} + \rho_\protp F_{\mu_\protp}) \circ F_{\mu_\pa}^{-1}(\omega) 
\end{align*}
\end{corollary}
    
    
 

\paragraph*{A Note on Our Use of $\Wass_1$ and $\Wass_2$.}  In this work we make use of both $\Wass_1$ and $\Wass_2$.  Our use of $\Wass_1$ is restricted to our distributional parity calculations. This choice is motivated by the fact that in the special case when $\gamma=\UF_\PR$, the Wasserstein-1 distance recovers $\UF_\PR$.   On the other hand, we use $\Wass_2$ to compute barycenters since $\Wass_2$ is known to be strictly convex, and provided that some $\mu_\prot$ is non-atomic, for $p=2$ the barycenter which minimizes  Eq. \ref{def:barycenter} is unique \cite[Proposition 3.5]{agueh2011barycenters}.  
% It is worth noting that $\Wass_1(\mu,\nu) \leq \Wass_2(\mu,\nu)$ \cite{Villani2008OptimalTO}.  

% it is known to be strictly convex and the $\Wass_2$-barycenter, i.e. solution to Eq. (\ref{eq:barycenter}) when $p=2$, is known to be unique \cite{agueh2011barycenters}.  Under different assumptions, and for other choices in $p$, the barycenter may well defined, however uniqueness may be compromised, see \cite[Proposition 7.19]{santambrogio2015optimal} for more detail. 


 
